The Compact Linear Collider (CLIC) - Project Implementation Plan

The Compact Linear Collider (CLIC) is a TeV-scale high-luminosity linear $e^+e^-$ collider under development by international collaborations hosted by CERN. This document provides an overview of the design, technology, and implementation aspects of the CLIC accelerator. For an optimal exploitation of its physics potential, CLIC is foreseen to be built and operated in stages, at centre-of-mass energies of 380 GeV, 1.5 TeV and 3 TeV, for a site length ranging between 11 km and 50 km. CLIC uses a Two-Beam acceleration scheme, in which normal-conducting high-gradient 12 GHz accelerating structures are powered via a high-current Drive Beam. For the first stage, an alternative with X-band klystron powering is also considered. CLIC accelerator optimisation, technical developments, and system tests have resulted insignificant progress in recent years. Moreover, this has led to an increased energy efficiency and reduced power consumption of around 170 MW for the 380 GeV stage, together with a reduced cost estimate of approximately 6 billion CHF. The construction of the first CLIC energy stage could start as early as 2026 and first beams would be available by 2035, marking the beginning of a physics programme spanning 25-30 years and providing excellent sensitivity to Beyond Standard Model physics, through direct searches and via a broad set of precision measurements of Standard Model processes, particularly in the Higgs and top-quark sectors.

==> 0.00-Preamble/Author_List.tex <==
%Australia, Melbourne
%Accelerator
%email Mark Boland <Mark.Boland@lightsource.ca>
%dated 17/09/2018
%email Professor Geoffrey Taylor <gntaylor@unimelb.edu.au>
%dated 02/10/2018
\addauthor{
% M.J.~Boland, % removed, moved institute
% U.~Felzmann, % removed
T.K.~Charles, % added, from Monash Univ.
P.J.~Giansiracusa,
T.G.~Lucas,
R.P.~Rassool,
M.~Volpi$^{1}$\\ % added
\emph{University of Melbourne, Melbourne, Australia}
}

%Australia, Melbourne, Monash
%Accelerator
%email Professor Geoffrey Taylor <gntaylor@unimelb.edu.au>
%dated 02/10/2018
\addauthor{
C.~Balazs\\
% T.K.~Charles\\ % removed, to Univ of Melbourne
\emph{Monash University, Melbourne, Australia}
}

%Belarus, Sosny
%Accelerator
\addauthor{
A.~Patapenka, 
I.~Zhuk\\
\emph{Joint Institute for Power and Nuclear Research - Sosny, Minsk, Belarus}
}

%Canada, Saskatchewan
%Accelerator
%email Mark Boland <Mark.Boland@lightsource.ca>
%dated 17/09/2018
\addauthor{
M.J.~Boland\\ % added
\emph{University of Saskatchewan, Saskatoon, Canada}
}

%China., Beijing, IHEP
%Accelerator
\addauthor{
Y.~Chi,
X.~He,
G.~Pei,
S.~Pei,
G.~Shu,
X.~Wang,
J.~Zhang,
F.~Zhao,
Z.~Zhou\\
\emph{Institute of High Energy Physics, Beijing, China}
}

%China, Beijing, Tsinghua
%Accelerator
%email Jiaru Shi <shij@tsinghua.edu.cn>
%dated 27/09/2018
\addauthor{
H.~Chen,
Y.~Gao,
W.~Huang,
Y.P.~Kuang,
B.~Li,
Y.~Li,
X.~Meng, % added
J.~Shao,
J.~Shi,
C.~Tang,
P.~Wang, % added
X.~Wu,
H.~Zha\\ % added, was at CERN
\emph{Tsinghua University, Beijing, China}
}

%China, Shandong
%Accelerator
\addauthor{
L.~Ma,
Y.~Han\\
\emph{Shandong University, Jinan, China}
}

%China, Shanghai
%Accelerator
%email Zhentang <zhaozhentang@sinap.ac.cn>
%dated 27/09/2018
\addauthor{
W.~Fang,
Q.~Gu, 
D.~Huang, 
X.~Huang, 
J.~Tan, 
Z.~Wang, 
Z.~Zhao\\
\emph{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai, China}
}

%Denmark, Aarhus
%Accelerator
%email Ulrik Ingerslev Uggerhøj <ulrik@phys.au.dk>
%dated 06/09/2018
\addauthor{
U.~Uggerh{\o}j, % updated name to o-slash
T.N.~Wistisen\\
\emph{Aarhus University, Aarhus, Denmark}
}

%Estonia, Tartu
%Accelerator
%email Vahur Zadin <vahur.zadin@ut.ee>
%dated 27/09/2018
\addauthor{
A.~Aabloo,
R.~Aare, % added
% K.~Eimre, % removed
K.~Kuppart,
S.~Vigonski,
V.~Zadin\\
\emph{University of Tartu, Tartu, Estonia}
}

%Finland, Helsinki
%Accelerator
%email Österberg, Kenneth <kenneth.osterberg@helsinki.fi>
%dated 27/09/2018
\addauthor{
M.~Aicheler,
E.~Baibuz,
E.~Br\"{u}cken,
F.~Djurabekova$^{2}$,
P.~Eerola$^{2}$,
F.~Garcia,
E.~Haeggstr\"{o}m$^{2}$,
K.~Huitu$^{2}$,
V.~Jansson$^{2}$,
% V.~Karimaki, % removed
I.~Kassamakov$^{2}$,
J.~Kimari$^{2}$, % added
A.~Kyritsakis,
S.~Lehti,
A.~ Meril\"{a}inen$^{2}$,
R.~Montonen$^{2}$,
% T.~Niinikoski, % removed
K.~Nordlund$^{2}$,
K.~\"{O}sterberg$^{2}$,
% M.~Parekh$^{3,4}$, % removed
A.~Saressalo, % added
% N.A.~T\"{o}rnqvist, % removed
J.~V\"{a}in\"{o}l\"{a},
M.~Veske\\
\emph{Helsinki Institute of Physics, University of Helsinki, Helsinki, Finland}
}

%France, CEA
%Accelerator
%email NAPOLY Olivier <Olivier.Napoly@cea.fr>
%dated 06/09/2018
\addauthor{
W.~Farabolini,
A.~Mollard,
% O.~Napoly,	% removed
F.~Peauger$^{3}$,	% RR: added now at CERN
J.~Plouin\\
\emph{CEA, Gif-sur-Yvette, France}
}

%France, LAL
%Accelerator
%email Philip Bambade <bambade@lal.in2p3.fr>
%dated 02/10/2018, 03/10/2018
\addauthor{
P.~Bambade,
I.~Chaikovska,
R.~Chehab,
N.~Delerue, % added
M.~Davier,
A.~Faus-Golfe, % added
A.~Irles, % added
W.~Kaabi,
% E.~Kou, % removed
F.~LeDiberder,
R.~P\"{o}schl,
D.~Zerwas\\
\emph{Laboratoire de l'Acc\'{e}l\'{e}rateur Lin\'{e}aire, Universit\'{e} de Paris-Sud XI, IN2P3/CNRS, Orsay, France}
}

%France, Annecy
%Accelerator
%email Max Chefdeville <chefdevi@lapp.in2p3.fr>
%dated 10/10/2018
\addauthor{
B.~Aimard,
G.~Balik,
% J.-P.~Baud, % removed
J.-J.~Blaising,
L.~Brunetti,
M.~Chefdeville,
A.~Dominjon, % added
C.~Drancourt,
N.~Geoffroy,
J.~Jacquemier,
A.~Jeremie,
Y.~Karyotakis,
J.M.~Nappa,
M.~Serluca, % added
S.~Vilalte,
G.~Vouters\\
\emph{LAPP, Universit\'{e} de Savoie, IN2P3/CNRS, Annecy, France}
}

%Germany, KIT Karlshruhe
%Accelerator
%email Axel Bernhard <axel.bernhard@kit.edu>
%dated 17/09/2018
\addauthor{
A.~Bernhard, % corrected spelling (h was missing)
S.~Casalbuoni, % added
S.~Hillenbrand, % added
J.~Gethmann, % added
A.~Grau, % added
E.~Huttel, % added
I.~Peric,
P.~Peiffer$^{4}$\\ % added
\emph{Karlsruhe Institute of Technology (KIT), Karlsruhe, Germany} % corrected spelling
}

%Greece, HEP-NTUA 
%Accelerator
%email Evangelos Gazis <Evangelos.Gazis@cern.ch>
%dated 06/09/2018
\addauthor{
T.~Alexopoulos,
T.~Apostolopoulos$^{5}$,  % added
E.N.~Gazis,
N.~Gazis,
% E.~Ikarios, % removed
V.~Kostopoulos$^{6}$,
S.~Kourkoulis\\
\emph{National Technical University of Athens, Athens, Greece}
}

%Hungary, Mining and Geological Survey
%Accelerator
%email Heilig Balázs <heilig.balazs@mbfsz.gov.hu>
%dated 23/11/2018
\addauthor{
B.~Heilig\\
\emph{Department of Basic Geophysical Research, Mining and Geological Survey of Hungary, Tihany, Hungary}
}

%Hungary
%Accelerator
%email Heilig Balázs <heilig.balazs@mbfsz.gov.hu>
%dated 23/11/2018
\addauthor{
J.~Lichtenberger\\
\emph{Space Research Laboratory, E\"otv\"os Lor\'and University, Budapest, Hungary}
}

%India, Indore
%Accelerator
%email Dr. Prasad A. Naik <panaik@rrcat.gov.in>
%dated 28/09/2018
\addauthor{
% P.D.~Gupta, % removed
P.~Shrivastava\\
\emph{Raja Ramanna Centre for Advanced Technology, Department of Atomic Energy, Indore, India}
}

%Iran, IPM
%Accelerator
%email Hessamaddin Arfaei <Hessamaddin.Arfaei@cern.ch>
%dated 27/09/2018
\addauthor{
% H.~Arfaei, % removed
M.K.~Dayyani,
H.~Ghasem$^{1}$,
S.S.~Hajari,
H.~Shaker$^{1}$\\
\emph{The School of Particles and Accelerators, Institute for Research in Fundamental Sciences, Tehran, Iran}
}

%Israel, Jerusalem, Racah
%Accelerator
%email Yinon Ashkenazy <yinonashkenazy@gmail.com>
%dated 06/09/2018
\addauthor{
Y.~Ashkenazy,
I.~Popov,	% added
E.~Engelberg, % added
A. Yashar\\	% added
\emph{Racah Institute of Physics, Hebrew University of Jerusalem, Jerusalem, Israel}
}

%Italy, INFN Frascati
%Accelerator
%email Andrea Ghigo <andrea.ghigo@lnf.infn.it>
%dated 10/09/2018 16:46
%dated 10/09/2018 17:51
\addauthor{
D.~Alesini,
M.~Bellaveglia,
B.~Buonomo,
A.~Cardelli,
M.~Diomede,
M.~Ferrario,
A.~Gallo,
A.~Ghigo,
A.~Giribono,
L.~Piersanti,
A.~Stella,
C.~Vaccarezza\\
\emph{INFN e Laboratori Nazionali di Frascati, Frascati, Italy}
}

%Italy, Trieste
%Accelerator
%email Gerardo D'Auria <gerardo.dauria@elettra.eu>
%dated 12/10/2018
\addauthor{
G.~D'Auria, 
S.~Di Mitri\\
\emph{Elettra Sincrotrone Trieste, Trieste, Italy}
}

%Japan, Tsukuba
%Accelerator
%email higo <higo@post.kek.jp>
%dated 28/09/2018
\addauthor{
T.~Abe, 
A.~Aryshev,
M.~Fukuda, % added
K.~Furukawa, % added 
H.~Hayano, % added
Y.~Higashi, % added
T.~Higo,
K.~Kubo, % added
S.~Kuroda, % added
% Y.~Makida, % removed
S.~Matsumoto, 
S.~Michizono, % added
T.~Naito, % added
T.~Okugi, % added
T.~Shidara, 
% T.~Takatomi, % removed
% Y.~Takubo, % removed
T.~Tauchi, 
N.~Terunuma, % added
% N.~Toge, % removed
% K.~Ueno, % removed
J.~Urakawa, 
A.~Yamamoto$^{1}$\\
% M.~Yamanaka\\ % removed
\emph{High Energy Accelerator Research Organization, KEK, Tsukuba, Japan}
}

%Madagascar, Antananarivo
%Accelerator
%email RABOANARY Roland <r_raboanary@yahoo.fr>
%dated 29/09/2018
\addauthor{
R.~Raboanary\\
\emph{University of Antananarivo, Antananarivo, Madagascar}
}

%Netherlands, Eindhoven
%Accelerator
%email Steinar Stapnes
%dated 23/11/2018
\addauthor{
O.J.~Luiten,
X.F.D.~Stragier\\
\emph{Eindhoven University of Technology, Eindhoven, Netherlands}
}

%Netherlands, Nikhef 
%Accelerator
%email stan.bentvelsen <stan.bentvelsen@nikhef.nl>
%dated 02/10/2018
\addauthor{
R.~Hart,
H.~van der Graaf\\
\emph{Nikhef, Amsterdam, Netherlands}
}

%Norway, Oslo
%Accelerator
%email Erik Adli <Erik.Adli@cern.ch>
%dated 06/09/2018
%dated 24/10/2018
\addauthor{
E.~Adli$^{1}$,
C.A.~Lindstr{\o}m, % added
R.~Lillest\o{}l,
L.~Malina$^{1}$,
J.~Pfingstner,
K.N.~Sjobak$^{1}$\\
\emph{University of Oslo, Oslo, Norway}
}

%Pakistan, Islamabad
%Accelerator
%email Hafeez Hoorani <hafeez.hoorani@cern.ch>
%dated 28/09/2018
\addauthor{
A.~Ahmad, % added
% W.~Ahmed, % removed
% M.I.~Asghar, % removed
H.~Hoorani,
W.A.~Khan\\ % added
\emph{National Centre for Physics, Islamabad, Pakistan}
}

%Poland, Cracow 2
%Accelerator
%email Pawel Bruckman De Renstrom <Pawel.Bruckman.de.Renstrom@cern.ch>
%dated 08/10/2018
\addauthor{
P.~Br\"{u}ckman~de~Renstrom, % added
% W.~Daniluk, % removed
B.~Krupa,
M.~Kucharczyk,
T.~Lesiak,
% A.~Moszczynski, % removed
B.~Pawlik,
P.~Sopicki,
T.~Wojto\'{n},
L.~Zawiejski\\ 
\emph{Institute of Nuclear Physics PAN, Krakow, Poland }
}

%Russia, Dubna
%Accelerator
%email Grigory Shirkov <Grigory.Shirkov@cern.ch>
%dated 02/10/2018
\addauthor{
A.~Aloev,
N.~Azaryan,
J.~Budagov,
M.~Chizhov,
M.~Filippova,
V.~Glagolev,
A.~Gongadze,
S.~Grigoryan,
D.~Gudkov,
V.~Karjavine,
M.~Lyablin,
A.~Olyunin$^{1}$,
A.~Samochkine,
A.~Sapronov,
G.~Shirkov,
V.~Soldatov,
% A.~Solodko$^{1}$, % removed, now at CERN
E.~Solodko$^{1}$,
G.~Trubnikov,
I.~Tyapkin,
V.~Uzhinsky,
A.~Vorozhtov\\
\emph{Joint Institute for Nuclear Research, Dubna, Russia}
}

%Russia, BINP
%Accelerator
%email Eugene B. Levichev <E.B.Levichev@inp.nsk.su>
%dated 22/10/2018
\addauthor{
E.~Levichev,
N.~Mezentsev,
P.~Piminov,
D.~Shatilov,
P.~Vobly,
K.~Zolotarev\\
\emph{Budker Institute of Nuclear Physics, Novosibirsk, Russia}
}

%Russia, IAP
%Accelerator
%no authors

%Serbia, Belgrade
%Accelerator
%email Ivanka Bozovic <ibozovic@vin.bg.ac.rs>
%dated 06/09/2018
\addauthor{
I.~Bozovic-Jelisavcic,
G.~Kacarevic,
% S.~Lukic,	% removed
G.~Milutinovic-Dumbelovic,
M.~Pandurovic,
N.~Vukasinovic\\	% added
\emph{Vinca Institute of Nuclear Sciences, University of Belgrade, Belgrade, Serbia}
}

%South Korea
%Accelerator
%email Heilig Balázs <heilig.balazs@mbfsz.gov.hu>
%dated 23/11/2018
\addauthor{
Dong-Hun Lee\\
\emph{School of Space Research, Kyung Hee University, Yongin, Gyeonggi, South Korea}
}

%Spain, CELLS-ALBA
%Accelerator
%email Francis Perez <francis@cells.es>
%dated 07/09/2018
\addauthor{
N.~Ayala, % added
G.~Benedetti, % added
T.~Guenzel, % added
U.~Iriso,
Z.~Marti, % added
F.~Perez,
M.~Pont\\
\emph{CELLS-ALBA, Barcelona, Spain}
}

%Spain, Madrid, CIEMAT
%Accelerator
%email Toral Fernandez, Fernando <fernando.toral@ciemat.es>
%dated 06/09/2018
\addauthor{
% M.~Aguilar-Benitez, % removed
J.~Calero, 
M.~Dominguez,	% added
L.~Garcia-Tabares, 
D.~Gavela, 
% J.L.~Gutierrez, % removed
D.~Lopez, 
F.~Toral\\
\emph{Centro de Investigaciones Energ\'{e}ticas, Medioambientales y Tecnol\'{o}gicas (CIEMAT), Madrid, Spain}
}

%Spain, Spanish network, institute 3
%Accelerator
%email angeles.faus.golfe@gmail.com
%dated 04/10/2018
\addauthor{
% T.~Argyropoulos$^{1}$, % removed
C.~Blanch Gutierrez,
M.~Boronat,
D.~Esperante$^{1}$,
% A.~Faus-Golfe, % removed, on leave, also at LAL
J.~Fuster,
% N.~Fuster Martinez, % removed
% N.~Galindo Mu\~{n}oz, % removed
% I.~Garc\'{\i}a, % removed
B.~Gimeno, % added
% J.~Giner Navarro$^{1}$, % removed
P.~Gomis, % added
D.~Gonz\'{a}lez, % added
M.~Perell\'{o}, % added
E.~Ros,
M.A.~Villarejo, % added
A.~Vnuchenko, % added
M.~Vos\\
\emph{Instituto de F\'{\i}sica Corpuscular (CSIC-UV), Valencia, Spain}
}

%Spain, Vigo
%Accelerator
%no authors

%Sweden, Uppsala
%Accelerator
%email Tord Ekelöf <tord.ekelof@physics.uu.se>
%dated 06/09/2018
%updated 06/12/2018 (marked %RR / Roger Ruber)
\addauthor{
Ch.~Borgmann, % added %RR
R.~Brenner,
T.~Ekel\"{o}f, 
M.~Jacewicz,  
% J.~\"{O}gren , % removed, now at CERN
M.~Olveg{\aa}rd, 
R.~Ruber, 
V.~Ziemann\\
\emph{Uppsala University, Uppsala, Sweden}
}

%Switzerland, CERN
%Accelerator & Physics
%email Roberto Corsini <Roberto.Corsini@cern.ch>
%dated 05/11/2018
%updated 23/11/2018 (2x)
%updated 28/11/2018 (2x, marked %RC and %AA)
\addauthor{
D.~Aguglia,
J.~Alabau Gonzalvo % added %RC
M.~Alcaide Leon, % added
% N.~Alipour Tehrani$^7$, % removed
M.~Anastasopoulos, % added %RC
A.~Andersson, %RC
F.~Andrianala$^{7}$,
F.~Antoniou,
A.~Apyan, % added %RC
K.~Artoos,
S.~Assly, % added %AA
S.~Atieh,
C.~Baccigalupi, % added %RC
% R.~Ballabriga Sune, % removed
D.~Banon Caballero, % added %AA
M.J.~Barnes,
J.~Barranco Garcia,
A.~Bartalesi, % added %RC
% H.~Bartosik, % removed
J.~Bauche, % added
C.~Bayar, % added, PhD student from Ankara
C.~Belver-Aguilar,
A.~Benot Morell$^{8}$,
D.R.~Bett,
S.~Bettoni$^{9}$, %RC now at PSI (but did not work there for CLIC)
M.~Bettencourt, % added %RC
B.~Bielawski, % added %RC
% G.~Blanchot, % removed
O.~Blanco Garcia,
N.~Blaskovic Kraljevic, % added
L. Bobb$^{10}$, % added
B.~Bolzon$^{11}$, % added
X.A.~Bonnin,
D.~Bozzini, % added
E.~Branger, % added %RC
O.~Brunner,
H.~Burkhardt,
H.~Bursali, % added %RC
D.~Caiazza, % added %RC
S.~Calatroni, 
% M.~Campbell, % removed
B.~Cassany, % added %AA
E.~Castro, % added %AA
N.~Catalan Lasheras,
R.H.~Cavaleiro Soares, % added %RC
M.~Cerqueira Bastos,
A.~Cherif,
E.~Chevallay,
V.~Cilento$^{12}$, % added
B.~Constance, %RC
R.~Corsini, 
R.~Costa$^{13}$, % added
% B.~Cure, % removed
S.~Curt,
% B.~Dalena$^{11}$, % removed
A.~Dal Gobbo, % added %RC
% D.~Dannheim, % removed
E.~Daskalaki, % added %RC
L.~Deacon, % added %RC
A.~Degiovanni, % added %RC
G.~De Michele,
L.~De Oliveira,
% N.~Deelen, % removed
V.~Del Pozo Romano, % added
J.P.~Delahaye,
D.~Delikaris, % added
T.~Dobers,
S.~Doebert,
I.~Doytchinov, % added %RC
M.~Draper,
% F.~Duarte Ramos, % removed
A.~Dubrovskiy, %RC
M.~Duquenne, % added %RC
K.~Elsener,
J.~Esberg,
M.~Esposito,
V.~Fedosseev,
P.~Ferracin,
% A.~Fiergolski, % removed
K.~Foraz,
A.~Fowler,
F.~Friebel,
J-F.~Fuchs,
% C.A.~Fuentes Rojas, % removed
A.~Gaddi,
D.~Gamba, % added, was at Oxford
L.~Garcia Fajardo$^{14}$,
H.~Garcia Morales,
C.~Garion,
M.~Gasior, % added
L.~Gatignon,
J-C.~Gayde,
A.~Gerbershagen, % added %RC
H.~Gerwig,
G.~Giambelli, % added %RC
A.~Gilardi, % added %RC
A.N.~Goldblatt,
S.~Gonzalez Anton, % added
% C.~Grefe$^{13}$, % removed
A.~Grudiev,
F.G.~Guillot-Vignot,
M.L.~Gutt-Mostowy,
% M.~Hauschild, % removed
M.~Hein Lutz, % added %RC
C.~Hessler,
J.K.~Holma,
E.B.~Holzer, % modified, added middle name (B.)
M.~Hourican,
% D.~Hynds, % removed
E.~Ikarios, % added %RC
Y.~Inntjore Levinsen,
S.~Janssen, % added %RC
% B.~Jeanneret, % removed
A.~Jeff, % added
E.~Jensen,
M.~Jonker,
S.W.~Kamugasa, % added %RC
M.~Kastriotou,
J.M.K.~Kemppinen,
R.B.~Kieffer,
V.~Khan, % added %RC
% W.~Klempt, % removed
N.~Kokkinis, % added %AA
O.~Kononenko, %RC
A.~Korsback,
I.~Kossyvakis, % added %RC
Z.~Kostka, % added %RC
E.~Koukovini Platia,
J.W.~Kovermann, %RC
C-I.~Kozsar,
% I.~Kremastiotis$^{14}$, % removed
% S.~Kulis, % removed
A.~Latina,
F.~Leaux,
P.~Lebrun,
T.~Lefevre,
% L.~Linssen, % removed
X.~Liu, % added
% X.~Llopart Cudie, % removed
S.~Magnoni, % added %RC
C.~Maidana, % added %RC
% A.A.~Maier, % removed
H.~Mainaud Durand,
S.~Mallows, % added %RC
E.~Manosperti,
C.~Marelli,
E.~Marin Lacoma,
C.~Marrelli, % added %RC
S.~Marsh, % added
R.~Martin,
I.~Martini, % added %RC
M.~Martyanov, % added %RC
S.~Mazzoni,
G.~Mcmonagle,
% O.~Mete, % removed
L.M.~Mether,
C.~Meynier, % added %RC
M.~Modena,
A.~Moilanen, % added %RC
R.~Mondello, % added %RC
P.B.~Moniz Cabral, % added
N.~Mouriz Irazabal, % added %RC
% R.M.~M\"{u}nker$^{15}$, % removed
T.~Muranaka,
J.~Nadenau, % added
J.G.~Navarro, % added
J.L.~Navarro Quirante, % added %RC
E.~Nebot Del Busto,
% N.~Nikiforou,
P.~Ninin, % added
% D.~Nisbet, % removed
% J-M.~Nonglaton, % removed
M.~Nonis, % added
% F.X.~Nuiry, % removed
% A.~N\"{u}rnberg, % removed
J.~\"{O}gren , % added, was at Uppsala
% M.~Olvegard, % removed, double listing, now at Uppsala
A.~Olyunin, % added %RC
J.~Osborne,
A.C.~Ouniche, % added %RC
R.~Pan$^{15}$, % added
S.~Papadopoulou,
Y.~Papaphilippou,
G.~Paraskaki, % added %RC
A.~Pastushenko$^{12}$, % added
A.~Passarelli,
M.~Patecki,
L.~Pazdera,
D.~Pellegrini,
K.~Pepitone,
% E.~Perez Codina, % removed
A.~Perez Fontenla,
T.H.B.~Persson,
S.~Pitman, % added
% M.~Petri\v{c}, % removed
% F.~Pitters$^{16}$, % removed
S.~Pittet,
F.~Plassard,
D.~Popescu, % added %RC
% R.~Rajamak, % removed
R.~Rajamaki, % added
% S.~Redford$^{10}$, % removed
L.~Remandet, % added %RC
Y.~Renier$^{15}$,
S.F.~Rey,
G.~Riddone,
% L.~Rinolfi, % removed
E.~Rodriguez Castro,
% P.~Roloff, % removed
C.~Rossi,
F.~Rossi, % added %RC
V.~Rude,
I.~Ruehl, % added
G.~Rumolo,
% A.~Sailer, % removed
J.~Sandomierski % added %RC
% E.~Santin, % removed
C.~Sanz, % added %RC
J.~Sauza Bedolla, % added
% D.~Schlatter, % removed
H.~Schmickler,
D.~Schulte,
E.~Senes, % added %RC
C.~Serpico, % added %AA
G.~Severino, % added %RC
N.~Shipman,
% E.~Sicking, % removed
% R.~Simoniello, % removed
P.K.~Skowronski,
P.~Sobrino Mompean,
L.~Soby,
P.~Sollander, % added
A.~Solodko, % added, was at Dubna, Russia
M.P.~Sosin,
% S.~Sroka, % removed
S.~Stapnes,
G.~Sterbini,
G.~Stern, % added %RC
% R.~Str\"{o}m, % removed
M.J.~Stuart, % added
I.~Syratchev,
K.~Szypula, % added
F.~Tecker,
P.A.~Thonet,
P.~Thrane, % added %RC
L.~Timeo,
H.~Timko,
M.~Tiirakari, % added
R.~Tomas Garcia,
C.I.~Tomoiaga, % added %RC
% P.~Valerio$^{18}$, % removed
A.L.~Vamvakas,
J.~Van Horne, % added %RC
N.~Vitoratou, % added %RC
% A.~Vivoli, % removed
V.~Vlachakis, % added %RC
% M.A.~Weber, % removed
R.~Wegner,
M.~Wendt,
M.~Widorski, % added
O.E.~Williams, % added
B.~Woolley
W.~Wuensch,
J.~Uythoven,
A.~Xydou, % added %RC
% A.~Yamamoto, % added, but already listed under KEK, Japan
R.~Yang, % added
A.~Zelios, % added %RC
% H.~Zha, % removed, moved to Tsinghua, China
Y.~Zhao$^{16}$, % added
M.~Zingl, % added %RC
P.~Zisopoulos\\
\emph{CERN, Geneva, Switzerland}
}

%Switzerland, Zurich
%Accelerator
%email Markus Rothacher <markus.rothacher@ethz.ch>
%dated 03/10/2018
\addauthor{
S.~Guillaume, % added
M.~Rothacher\\ % added
\emph{ETH Zurich, Institute of Geodesy and Photogrammetry, Zurich, Switzerland}
}

%Switzerland, Villigen, PSI
%Accelerator
%email Garvey Terence (PSI) <terence.garvey@psi.ch>
%dated 12/09/2018
\addauthor{
M.~Bopp,
H.H.~Braun,
P.~Craievich, %added
% M.~Csatari Divall, % removed
M.~Dehler,
T.~Garvey,
M.~Pedrozzi, % added
J.Y.~Raguin,
L.~Rivkin$^{17}$,
R.~Zennaro\\
\emph{Paul Scherrer Institut, Villigen, Switzerland}
}

%Turkey, Ankara
%Accelerator
%email Avni Aksoy <Avni.Aksoy@ankara.edu.tr> 
%dated 28/09/2018 (via Alexia)
\addauthor{
A.~Aksoy,
Z.~Nergiz$^{18}$,
% E.~Pilicer$^{21}$, % removed
% I.~Tapan$^{21}$, % removed
\"{O}.~Yavas\\
%\emph{IAT, Ankara University, Ankara, Turkey}
\emph{Ankara University, Ankara, Turkey}
}

%Ukraine, IAP-NASU 
%Accelerator
%email Volodymyr Storizhko - IAP NASU <ipfmail@ipfcentr.sumy.ua>
%dated 10/09/2018
\addauthor{
V.~Baturin,
O.~Karpenko, % added
R.~Kholodov,
O.~Lebed, % added
S.~Lebedynskyi,
% V.~Miroshnichenko, % removed
S.~Mordyk,
I.~Musienko, %added
Ia.~Profatilova, % $^{1}$, updated
V.~Storizhko\\
\emph{Institute of Applied Physics, National Academy of Sciences of Ukraine, Sumy, Ukraine}
}

%UK, Dundee
%Accelerator
%email Allan Gillespie (Staff) <W.A.Gillespie@dundee.ac.uk>
%dated 02/10/2018
\addauthor{
W.A.~Gillespie\\
% R.~Pan, % removed
% M.A~Tyrk\\ % removed
\emph{University of Dundee, Dundee, United Kingdom}
}

%UK, Edinburgh
%Accelerator
%email Heilig Balázs <heilig.balazs@mbfsz.gov.hu>
%dated 23/11/2018
\addauthor{
C.~Beggan\\
\emph{British Geological Survey, Edinburgh, United Kingdom}
}

%UK, Lancaster
%Accelerator
%email Dexter, Amos <a.dexter@lancaster.ac.uk>
%dated 02/10/2018
\addauthor{
R.J.~Apsimon$^{19}$,
I.~Bailey$^{19}$,
G.C.~Burt$^{19}$,
% D.~Constable$^{19}$, % removed
A.C.~Dexter$^{19}$,
A.V.~Edwards$^{19}$, % added
V.~Hill$^{19}$, % added
W.L.~Millar$^{19}$, % added
% S.~Karimian$^{19}$, % removed
% C.~Lingwood$^{19}$\\ % removed
K.~Papke$^{19}$\\ % added
\emph{Lancaster University, Lancaster, United Kingdom}
}

%UK, London 1
%Accelerator
%email Karataev, Pavel <Pavel.Karataev@rhul.ac.uk>
%dated 28/09/2018
%updated 19/11/2018
\addauthor{
T.~Aumeyr, % added
L.~Bobb, % added
A.~Bosco, 
S.~Boogert, % from London 2
G.~Boorman, % from London 2
F.~Cullinan, % added
S.~Gibson, % from London 2
P.~Karataev,
K.~Kruchinin, % removed then added
K.~Lekomtsev, 
A.~Lyapin, % from London 2
L.~Nevay, 
W.~Shields, % from London 2
J.~Snuverink, % removed then added
J.~Towler, % added
E.~Yamakawa\\ % removed then added
\emph{The John Adams Institute for Accelerator Science, Royal Holloway, University of London, Egham, United Kingdom}
}

%UK, London 2
%Accelerator
% email Karataev, Pavel <Pavel.Karataev@rhul.ac.uk>
% dated 28/09/2018
\addauthor{
V.~Boisvert,
% S.~Boogert, % moved to London 1
% G.~Boorman, % moved to London 1
% S.~Gibson, % moved to London 1
% A.~Lyapin, % moved to London 1
% W.~Shields, % moved to London 1
% P.~Teixeira-Dias, % removed
S.~West\\
\emph{Royal Holloway, University of London, Egham, United Kingdom}
}

%UK, Manchester
%Accelerator
%email roger.jones@manchester.ac.uk
%confirmed email reception
\addauthor{
R.~Jones,
N.~Joshi\\
\emph{University of Manchester, Manchester, United Kingdom}
}

%UK, Oxford
%Accelerator
%email Philip Burrows <philip.burrows@physics.ox.ac.uk>
%dated 09/09/2018
\addauthor{
D.~Bett, % added
R.M.~Bodenstein$^{1}$, % updated, also at CERN      % added middle name (M.)
T.~Bromwich,
P.N.~Burrows$^{1}$, % updated, also at CERN
G.B.~Christian$^{10}$, % updated, now at Diamond
% D.~Gamba$^{1}$, % removed, now at CERN
C.~Gohil$^{1}$, % added
P.~Korysko$^{1}$, % added
J.~Paszkiewicz$^{1}$, % added
C.~Perry,
R.~Ramjiawan, % added
J.~Roberts\\ % updated, removed also at CERN
\emph{John Adams Institute, Department of Physics, University of Oxford, Oxford, United Kingdom}
}

%UK, Warrington, Daresbury
%Accelerator
%email Jim Clarke - UKRI STFC <jim.clarke@stfc.ac.uk>
%dated 06/09/2018
\addauthor{
A.~Bainbridge$^{19}$, % added
J.A.~Clarke$^{19}$,
% N.A.~Collomb, % removed
% S.P.~Jamison$^{19}$, % removed
N.~Krumpa,						% added
B.J.A.~Shepherd$^{19}$,
D.~Walsh$^{19}$\\
\emph{STFC Daresbury Laboratory, Warrington, United Kingdom}
}

%USA, Argonne
%Accelerator & Physics
%email Demarteau, Marcel <demarteau@anl.gov>
%dated 12/10/2018
\addauthor{
W.~Gai, % added (accelerator)
W.~Liu, % added (accelerator)
J.~Power\\ % added (accelerator)
\emph{Argonne National Laboratory, Argonne, USA}
}

%USA, Cornell
%Accelerator
%no authors

%USA, FNAL
%Accelerator
%email Nathan Eddy <eddy@fnal.gov>
%dated 28/09/2018
%no authors

%USA, JLAB
%Accelerator
%email Andrew Hutton <andrew@jlab.org>
%dated 27/09/2018
%no authors

%USA, Northwestern
%Accelerator
%no authors

%USA, Santa Cruz
%Accelerator
%no authors

%USA, SLAC
%Accelerator
%email Tantawi, Sami <tantawi@slac.stanford.edu>
%dated 13/09/2018
\addauthor{
C.~Adolphsen, 
T.~Barklow, 
% M.~Breidenbach, % removed
V.~Dolgashev, % added
M.~Franzi, % added
N.~Graf, 
J.~Hewett, 
M.~Kemp, % added
T.~Markiewicz, 
% D.~McCormick, % removed
K.~Moffeit, 
J.~Neilson, % added
Y.~Nosochkov,
M.~Oriunno, 
N.~Phinney, 
T.~Rizzo, 
S.~Tantawi, 
% F.~Wang, % removed
J.~Wang, 
B.~Weatherford % added
G.~White, 
M.~Woodley\\
\emph{SLAC National Accelerator Laboratory, Menlo Park, USA}
}


\addauthor{
\begin{flushleft}
{$^{1}$}Also at CERN, Geneva, Switzerland\\
{$^{2}$}Also at Department of Physics, University of Helsinki, Helsinki, Finland\\
{$^{3}$}Now at CERN, Geneva, Switzerland\\
{$^{4}$}Now at Johannes-Gutenberg University, Mainz, Germany\\
{$^{5}$}Also at Department of Informatics, Athens University of Business and Economics, Athens, Greece\\
{$^{6}$}Also at University of Patras, Patras, Greece\\
{$^{7}$}Also at University of Antananarivo, Antananarivo, Madagascar\\
{$^{8}$}Also at IFIC, Valencia, Spain\\
{$^{9}$}Now at PSI, Villigen, Switzerland\\
{$^{10}$}Now at Diamond Light Source, Harwell, United Kingdom\\
{$^{11}$}Now at CEA, Gif-sur-Yvette, France\\
{$^{12}$}Also at LAL, Orsay, France\\
{$^{13}$}Also at Uppsala University, Uppsala, Sweden\\
{$^{14}$}Now at LBNL, Berkeley CA, USA\\
{$^{15}$}Now at DESY, Zeuthen, Germany\\
{$^{16}$}Also at Shandong University, Jinan, China\\
{$^{17}$}Also at EPFL, Lausanne, Switzerland\\
{$^{18}$}Also at Omer Halis Demir University, Nigde, Turkey\\
{$^{19}$}Also at The Cockcroft Institute, Daresbury, United Kingdom\\

\end{flushleft}
}



==> 0.00-Preamble/Preamble.tex <==
Some stuff here we need for the preamble...



